Maps of toric varieties in Cox coordinates

The Cox ring provides a coordinate system on a toric variety analogous to the homogeneous coordinate ring of projective space. Rational maps between projective spaces are described using polynomials in the coordinate ring, and we generalise this to toric varieties, providing a unified description of arbitrary rational maps between toric arieties in terms of their Cox coordinates. Introducing formal roots of polynomials is necessary even in the simplest examples.

==> toricmapsexamples.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%%   EXAMPLES OF MAPS OF TORIC VARIETIES
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Computability and examples}
\label{sect:examples}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Cox coordinates and computability}

The main theorem gives an effective algorithm for computing
complete descriptions of rational maps. Given a description,
our results show how to determine the regularity locus of the
underlying map and how to calculate image and preimage of subschemes
in an algorithmic way.

We have not made a serious study of the complexity of these algorithms,
but it is easy to get an informal sense of where the computation lies.
The calculation of a map ring $\mapring{\Phi}$ and its generators $\mvsa_i$
is the only computationally expensive calculation that arises in this
general framework for describing maps between toric varieties that is
not already needed when describing maps between ordinary projective
spaces or products of them. It is clear from the constructive proofs of
existence that this only requires GCD calculations, so it shouldn't be
regarded as formidable. We have implemented this in the computational
algebra system {\sc Magma} \cite{magma}, and in practical examples it
seems that factorising polynomials in place of some GCDs is effective,
since the number of GCD calculations blows up with the number of
Cox coordinates---at first sight we need all pairwise GCDs.


\subsection{Further examples}

We do several blow ups and give their complete description.

\subsubsection{Three toric blow ups}

These are well-known examples where the use of radical expressions
is already entrenched. In our language, these radical weighted blow ups
are complete descriptions.

\paragraph{Standard blow up of $\CC^3 $ at the origin}
Let $X$ be the toric variety with Cox ring $\CC[x_1, x_2, x_3, x_4]$,
irrelevant ideal $B_X=(x_1,x_2,x_3)$ and grading $(1,1,1,-1)$.
The variety $X$ is the standard blow up of $\CC^3$
at the origin, and it has complete description:
\begin{align*}
X & \longrightarrow \CC^3\\
[x_1, x_2, x_3, x_4] & \longmapsto [x_1 x_4, x_2 x_4, x_3 x_4].
\end{align*}

\paragraph{Blow up of $\half(1,1,1)$ singularity}
Let $Y$ be the standard affine $\half(1,1,1)$ singularity:
$\cox Y = \CC[y_1,y_2,y_3]$ with trivial irrelevant ideal
and grading $\half(1,1,1)$.
The standard weighted blow up of the origin has domain $X$
with Cox ring $\cox X = \CC[x_1, x_2, x_3, x_4]$, irrelevant ideal $B_X=(x_1, x_2, x_3)$
and grading $(1,1,1,-2)$. The blow up has complete description:
\begin{align*}
X &\longrightarrow Y\\
[x_1, x_2, x_3, x_4] & \longmapsto [x_1 {x_4}^{\half}, x_2 {x_4}^{\half}, x_3 {x_4}^{\half}].
\end{align*}

\paragraph{Weighted blow ups of $\quarter(1,1,2)$ singularity}
Let $Y$ be the affine $\frac{1}{4}(1,1,2)$ singularity:
$\cox Y = \CC[y_1,y_2,y_3]$ with trivial irrelevant ideal
and grading $\frac{1}4(1,1,2)$.
The weighted blow up $bl_{(1,1,2)}$ of the origin has complete
description
\begin{align*}
X &\longrightarrow Y\\
[x_1, x_2, x_3, x_4] & \longmapsto [x_1 {x_4}^{\quarter}, x_2 {x_4}^{\quarter}, x_3 {x_4}^{\half}].
\end{align*}
where $X$ has $\cox X = \CC[x_1, x_2, x_3, x_4]$, irrelevant ideal $B_X=(x_1, x_2, x_3)$
and grading $(1,1,2,-4)$.





\subsubsection{Reading toric birational maps with complete descriptions}
\label{sect:example_toric_birational}

Let $X=\PP(1,1,2)$ with Cox coordinates $x_1, x_2, x_3$ and $Y$ be the toric
variety with Cox coordinates $y_1, y_2, y_3, y_4$, bi-grading given by the matrix
of weights
\[
\begin{pmatrix}
1&2&0&-1\\0&0&1&1
\end{pmatrix}
\quad
\text{and irrelevant ideal}
\quad
B_Y = (y_1,y_2) \cap (y_3,y_4).
\]
Suppose $X$ and $Y$ are described by fans in a common lattice $N=\ZZ^2$
as follows.
\makefan{
      \gavina
      {\ar (3,0); (5,0)};
      (8,0);(9,0):;
      \gavinb}
The implicit birational map between $X$ and $Y$ is
\begin{align*}
\varphi\colon X &\dashrightarrow Y
&\text{and}\quad
\psi\colon Y &\dashrightarrow X\\
[x_1, x_2, x_3] &\longmapsto [x_1,x_1 x_2, x_1 x_3, x_1 x_2] &
[y_1, y_2, y_3, y_4] &\longmapsto [{y_1}^2 y_4, y_2 y_4, y_1 y_2 y_3 y_4],
\end{align*}
for indeed the compositions are
\[
[x_1, x_2, x_3] \longmapsto
[x_1,x_1 x_2, x_1 x_3, x_1 x_2] \longmapsto
[{x_1}^3 x_2, {x_1}^2 {x_2}^2,{x_1}^4 {x_2}^2 x_3] = [x_1, x_2, x_3]
\]
and
\begin{align*}
[y_1, y_2, y_3, y_4] \longmapsto
[{y_1}^2 y_4, y_2 y_4, y_1 y_2 y_3 y_4] &\longmapsto
[{y_1}^2 y_4, {y_1}^2 y_2 {y_3}^2, {y_1}^3 y_2 y_3 {y_4}^2,{y_1}^2 {y_2} {y_4}^2]\\
& \phantom{\longmapsto} \ =
[{y_1}, y_2, {y_1}^3 y_2 y_3 {y_4}^2,{y_1}^3 {y_2} {y_4}^3] \\
& \phantom{\longmapsto} \ = [y_1, y_2, y_3, y_4],
\end{align*}
using the two rows of the gradings of $Y$ to simplify the
final expression in two steps.

The easiest way to confirm that the descriptions satisfy the
homogeneity and relevance conditions is to compare them to descriptions of
the same maps by rational functions:
$\varphi$ can be described by $\Phi=(1,x_2/ x_1,x_3/{x_1}^2,x_2/x_1)$
or by $\Phi=(1,x_2/x_1, 1, x_1 x_2/ x_3)$, which looks nicer but has
smaller regular locus $\Reg\Phi$ (but still a codimension~$1$ complement);
$\psi$ can be described by $\Psi=(1,y_2/{y_1}^2,y_2 y_3/({y_1}^3 y_4))$.

The geometry of this birational equivalence evident in the fans but it is
not clear from these descriptions. It is better seen using complete descriptions.
We can make complete descriptions easily from the original monomial
descriptions (which are both regular on the respective entire GIT covers).
The question is simply how much can we cancel. For $\varphi$ we
can use the first grading of $Y$ to remove a $\sqrt{x_1}$ factor,
and then the second grading to remove a further $x_1$: thus
\begin{align*}
[x_1,x_1 x_2, x_1 x_3, x_1 x_2] &\text{ becomes }
[\sqrt{x_1}, x_2, x_1 x_3, x_1 x_2 \sqrt{x_1}]\\
 & \text{ which in turn becomes }
[\sqrt{x_1}, x_2, x_3, x_2 \sqrt{x_1}].
\end{align*}
Similarly we can modify the description of $\psi$, so the result is
\begin{align*}
\varphi\colon [x_1, x_2, x_3] &\longmapsto [\sqrt{x_1}, x_2, x_3, x_2 \sqrt{x_1}]\\
\psi\colon [y_1, y_2, y_3, y_4] &\longmapsto [y_1^2 \sqrt{y_4},y_2 \sqrt{y_4}, y_1 y_2 y_3].
\end{align*}
Many features of the birational geometry are now clear.
The map $\varphi$ is not defined at the three $0$-strata of $X$,
while $\psi$ is not defined on the loci $\Supp(y_1) \cap \Supp(y_4)$
and $(y_2) \cap (y_4)$ in $Y$.
The coordinate loci $(x_1)$ and $(x_2)$ in $X$ are contracted,
and similarly $(y_1)$, $(y_2)$ and $(y_4)$ in $Y$ are contracted.
Furthermore, comparing with the weighted blow ups above, we see that
$(x_1)$ and $(y_4)$ are contracted as $\frac{1}2(1,1)$ exceptional divisors,
while $(y_1)$ is a $(2,1)$ weighted blow up of a smooth point,
and $(y_2)$ and $(x_2)$ are ordinary (smooth) blow ups of smooth points.


\subsubsection{Toric del Pezzo surface in a weighted projective 5-space}
\label{sect:example_del_pezzos_in_wps}


Fix two toric varieties $X$ and $Y$ and a map $\alpha\colon\Pic Y \to \Pic X$.
We can use the structure of descriptions to classify all the regular maps
$\varphi\colon X \to Y$ for which $\varphi^*=\alpha$.
We present an easy example to illustrate the technique.
For brevity, we will assume that the image of $\varphi$ is not contained
in any toric stratum of $Y$, not even after a change of coordinates on $Y$.

Let $X = \FF_1$, simply $\PP^2$ blown up in a single point,
a del Pezzo surface of degree $8$.
Thus
\[
\cox{X} = \CC[x_1, x_2, x_3, x_4]
\quad\text{graded by $\ZZ^2$ with gradings}\quad
 \begin{pmatrix}
   1&1&1&0\\
   0&0&1&1
 \end{pmatrix}
\]
and irrelevant ideal $(x_1,x_2) \cap (x_3,x_4)$.
Consider also $Y = \PP(1,1,1,2,2,2)$:
\[
\cox{Y} = \CC[y_1, y_2, y_3, y_4, y_5, y_6]
\quad\text{graded by $\ZZ$ with gradings}\quad
 \begin{pmatrix}
   1&1&1&2&2&2
 \end{pmatrix}.
\]

For the demonstration, we assume that the regular map $\varphi\colon X \to Y$
pulls back a divisor in $\ccO_Y(2)$ (the ample generator of $\Pic Y$)
to an anticanonical divisor of $X$ in $\ccO(3,2)$. We claim that in
such case the map $\varphi$ is unique up to changes of coordinates on
$X$ and $Y$. (This is analogous to nondegenerate quadratic maps
$\PP^1\rightarrow\PP^2$ boiling down to the usual conic: the nominated
linear systems in source and target have the same dimension in each case,
so the only concern for us is to handle the `de-Veronese' process on $Y$.)

So let $\Phi\colon \CC^4 \multito \CC^6$ be a complete description of $\varphi$.
By condition~\ref{item:complete_description_Cartier} the multivalued sections
$(\Phi^*y_1)^2$,
$(\Phi^*y_2)^2$,
$(\Phi^*y_3)^2$,
$\Phi^*y_4$,
$\Phi^*y_5$ and
$\Phi^*y_6$ are all single valued.
Applying the homogeneity condition~\ref{item:homogeneity_cond_on degree_0}
we see that $\frac{\Phi^*y_2}{\Phi^*y_1}$ and $\frac{\Phi^*y_3}{\Phi^*y_1}$
are also single-valued.
Corollary~\ref{cor:regularity_locus_from_complete_description} implies that
all the $\Phi^*y_i$ are regular.
Thus we can write
\begin{align*}
  \Phi\colon \CC^m & \multito \CC^n\\
                   x & \multimapsto [f_1 \sqrt{g}, f_2 \sqrt{g}, f_3 \sqrt{g}, f_4, f_5, f_6]
\end{align*}
for polynomials $f_i, g \in \cox X$.

Applying the homogeneity condition~\ref{item:homogeneity_cond_on degree_0}
once more to this general form of the description, we see that
\begin{gather*}
     \deg f_1 = \deg {f_2} =\deg {f_3},\\
     \deg f_4 = \deg {f_5} =\deg {f_6},\\
     \text{and}\quad 2 \deg f_1 + \deg g = \deg f_4 = (3,2).
\end{gather*}
The last condition narrows the possibilities for the multidegree
of $f_1$:
\[
  \deg f_1 \in \set{(0,0), (1,0),(0,1),(1,1)}.
\]
But the linear systems in multidegrees $(0,0), (1,0),(0,1)$ are small,
and allowing the degree of $f_1$ to be any those would force
the $3$ sections $f_1,f_2, f_3$ to be linearly dependent.
A suitable coordinate change on $Y$ would then transform (at least)
one of $f_1, f_2, f_3$ to $0$, presenting the image of $\varphi$
inside some toric stratum, which is exactly what our simplifying
assumption forbids. So $\deg f_1 = (1,1)$.

So $\deg g =(1,0)$, and changing coordinates on $X$ we may assume $g = x_1$.
Also the $\CC$-linear span of $f_1,f_2, f_3$ is equal to the span
$x_1 x_4, x_2 x_4, x_3$, so changing coordinates on $Y$ we may assume
\[
   f_1 = x_1 x_4,\quad f_2 = x_2 x_4 \quad\text{and}\quad f_3 = x_3.
\]
The linear system $(3,2)$ is spanned by the nine monomials:
\[
  {x_1} {x_3}^2, {x_2} {x_3}^2,
  {x_1}^2  {x_3} {x_4}, {x_1} {x_2}  {x_3} {x_4},  {x_2}^2  {x_3} {x_4},
  {x_1}^3 {x_4}^2, {x_1}^2 {x_2} {x_4}^2, {x_1} {x_2}^2 {x_4}^2, {x_2}^3 {x_4}^2.
\]
However if any of $f_4, f_5, f_6$ contains any summand divisible by $x_1$
then we can change the coordinates on $Y$ to get rid of this summand.
For instance if $f_4 = {x_2} {x_3}^2 +  {x_1} {x_2}  {x_3} {x_4}$, then
$f_4 - (f_2 \sqrt{g}) (f_3 \sqrt{g}) = {x_2} {x_3}^2$.
Therefore we might assume $f_4, f_5, f_6$ are contained in span of
$
  {x_2} {x_3}^2,
  {x_2}^2  {x_3} {x_4},
  {x_2}^3 {x_4}^2
$
and changing coordinates on $Y$ again we may assume
\[
   f_4 = {x_2} {x_3}^2,\quad
   f_5 = {x_2}^2  {x_3} {x_4} \quad\text{and}\quad
   f_6 = {x_2}^3 {x_4}^2.
\]
Thus every map $\varphi$ satisfying the assumptions can be written as
\begin{align*}
  \varphi \colon X & \longrightarrow Y\\
                 x & \longmapsto
	[x_1 x_4 \sqrt{x_1}, x_2 x_4 \sqrt{x_1}, x_3 \sqrt{x_1},
	      {x_2} {x_3}^2,  {x_2}^2  {x_3} {x_4},  {x_2}^3 {x_4}^2]
\end{align*}
in some homogeneous coordinates on $X$ and $Y$.


